VRBubble: Enhancing Peripheral Awareness of Avatars for People with Visual Impairments in Social Virtual Reality

Social Virtual Reality (VR) is growing for remote socialization and collaboration. However, current social VR applications are not accessible to people with visual impairments (PVI) due to their focus on visual experiences. We aim to facilitate social VR accessibility by enhancing PVI's peripheral awareness of surrounding avatar dynamics. We designed VRBubble, an audio-based VR technique that provides surrounding avatar information based on social distances. Based on Hall's proxemic theory, VRBubble divides the social space with three Bubbles -- Intimate, Conversation, and Social Bubble -- generating spatial audio feedback to distinguish avatars in different bubbles and provide suitable avatar information. We provide three audio alternatives: earcons, verbal notifications, and real-world sound effects. PVI can select and combine their preferred feedback alternatives for different avatars, bubbles, and social contexts. We evaluated VRBubble and an audio beacon baseline with 12 PVI in a navigation and a conversation context. We found that VRBubble significantly enhanced participants' avatar awareness during navigation and enabled avatar identification in both contexts. However, VRBubble was shown to be more distracting in crowded environments.

==> Sections/2-Related_Work-rewrite.tex <==
\section{Related Work}

\subsection{Sonification of Virtual Environments}
There has been extensive work done to convey and navigate virtual environments through the use of audio cues. Audio beacons have been used to convey object positions \cite{walker2006navigation,lokki2005navigation, maidenbaum2013increasing, sanchez1999virtual, sanchez1997hyperstories}, such as Walker and Lindsay's \cite{walker2006navigation} study of the efficacy of different types of beacons on guidance or navigation through a virtual space. Maidenbaum et al. \cite{maidenbaum2013increasing} sonified the distance between the PVI's avatar and the virtual object in front of him to facilitate navigation in a virtual space. AudioDoom~\cite{sanchez1999virtual, sanchez1997hyperstories} was an acoustic virtual environment that was navigable via spatial sound generated by virtual objects and events. It was designed for blind children to improve their cognitive skills, such as 3D perception. 

Prior work has also used audio to identify objects \cite{heuten2006sonification, oliveira2015games}. For example, de Oliveira et al recreated a virtual stage and placed instruments in the environment. Participants then used different music tracks to identify and locate instruments on the stage.

Signals and audio reflections have been used to create echolocation emulations \cite{waters2001bat, wilkerson2010maze, andrade2018echo}. For example, Andrade et al. \cite{andrade2018echo} enabled PVI to use echolocation to navigate a desktop-based virtual world, where the user's avatar can produce mouth-click or clap sounds by pressing a key on a keyboard and hear the sound reflected in the environment. However, the echolocation method was only used by a small amount of blind people. 

List/grid-based verbal descriptions have also been used to better select and learn about objects in the environment \cite{westin2004game, matsuo2016audible, nair2021navstick}. Terraformers \cite{Terraformers, westin2004game} was a virtual world game that was accessible to PVI. Audio-based orientation and navigation tools were also supported in this game, such as a voiced menu for nearby objects \cite{westin2004game}. Nair et al. also compared similar menu systems with their novel game controller-based navigation technique, allowing PVI to look around a virtual world by scrubbing the thumbstick on a game controller to different directions; the system then announced what were in that direction via spatial audio.

\subsection{Sonification of Real-world Environments}
Similar audio techniques have also been applied to real-world settings, such as the use of beacons to mark waypoints \cite{wilson2007swan, holland2002gps}. Wilson et al. created a wearable audio navigation system that tracked user position in order to provide audio feedback about waypoints and obstacles around their location \cite{wilson2007swan}.

Verbal descriptions have been used to inform users about landmark locations and features to enhance awareness of the environment \cite{sato2019assist, gleason2018footnote}. Sato et al. placed physical beacons at landmarks to assist PVI in navigation while also providing descriptions of nearby landmarks.

Auditory icons have also been used to identify points of interest \cite{may2020spotlights, presti2019watchout}. May et al. examined approaches and recommendations for utilizing auditory icons to assist the user in forming cognitive maps while avoiding information overload \cite{may2020spotlights}.

Echolocation/sonar systems have also been utilized for real-world settings \cite{vera2014cane, fakhrhosseini2014listen}. Vera et al. utilized a smartphone and laser pointer to scan the environment. Distances between the user and the scanned element were then sonified.

\subsection{Specialized VR for People with Visual impairments}
Researchers have been working on accessible virtual experiences specialized for PVI for decades. Various virtual games have been created specifically for PVI, for example, Shades of Doom \cite{ShadeofDoom} and A Hero's Call \cite{AHeroCall}. When playing these games, PVI needed to use shortcut keys on the keyboard to control the movement of their avatars and receive spatial audio from the environment, such as sounds for space and object changes \cite{AHeroCall}. Besides desktop-based virtual games, some VR games have been designed, allowing PVI to interact with the virtual space via physical body movements. For example, Blind Swordsman \cite{BlindSwordsman} was a VR game on mobile devices, where a blind user can hear the spatial audio from the enemies, physically turn to that direction, and tap the touchscreen to swing his sword in the direction he is facing. Recently, Wedoff et al. designed a virtual reality game, called Virtual Showdown \cite{wedoff2019virtual}. PVI played the game by hitting a virtual ball into the opponent' goal across a virtual table using a bat. In this game, a Kinect was used to track the user's movement. A visually impaired user can thus hold a Nintendo Switch controller as the bat and receive both audio and vibration feedback to perceive the relative position of the ball from his bat.

Beyond gaming, some specialized virtual environments were created to train PVI on their real-world skills \cite{merabet2009audio, sanchez2006assisting, sanchez1999virtual}. For example, AudioDoom~\cite{sanchez1999virtual, sanchez1997hyperstories} was an acoustic virtual environment that was navigable via spatial sound generated by virtual objects and events. It was designed for blind children to improve their cognitive skills, such as 3D perception.  
%their cognitive , where “sound spectral cues” are developed to notice blind children of events such as 'door opening'. 
AudioMetro~\cite{audioMetro} was a similar virtual environment that simulated the urban subway system in Santiago, Chile, which enabled PVI to familiarize themselves with the real subway systems and better prepare for real world navigation. 
%Blind users were able to navigate the real-life transit system with greater confidence and develop a better mental model after using this audio-based .
Some researchers also leveraged external devices to generate virtual information for PVI to help them learn physical objects and spaces \cite{lahav2004exploration, jansson1999haptic, schloerb2010blindaid, sato2019assist}. For example, Jansson et al. \cite{jansson1999haptic} enabled PVI to use the stylus on a Phantom Premium device to "touch" a virtual space and receive force feedback to perceive different virtual surfaces and objects. Scholoerb et al. \cite{schloerb2010blindaid} also used the Phantom device but generated a haptic virtual environment that supported orientation and mobility training by simulating physical environments. Moreover, Lahav and Mioduser \cite{lahav2004exploration} enabled PVI to learn unknown environment by exploring haptic virtual spaces via a joystick. Sato et al. \cite{sato2019assist} placed Bluetooth beacons throughout a physical space to assist in verbal guidance navigation, as well as to better inform users about features and points of interest in their surroundings.
%Such haptic virtual environments were designed to help PVI learn graphs, shapes, and real-world environments. 

\subsection{Accessibility of Mainstream VR}
Compared to the aforementioned specialized VR, mainstream technology usually has lower cost, increased availability, and higher social acceptability \cite{shinohara2011shadow}. %As VR becomes increasingly used for social and collaborative purposes, it is critical to make the mainstream VR platforms accessible to guarantee PVI's equal access to potential resources and opportunities. 
Researchers have started investigating the accessibility of mainstream VR applications for PVI. 
%Some effort was made to make the mainstream \textit{desktop-based virtual worlds} accessible to PVI. 
%Here, desktop-based virtual worlds refer to simulated environments that are rendered on 2D computer screens and can be accessed via mouse, keyboard, and other desktop-mounted equipment such as joystick \cite{sousa2009head}.
%One typical example is the Second Life virtual community launched in 2003, which is often regarded as the first desktop-based virtual world \cite{SecondLife}. %with one million active users by 2013 [REF]. 
%Users of Second Life access to the platform from personal computers; they can build virtual structures, interact with other users, and even shop and trade virtual goods.
For example, Second Life was the first desktop-based virtual world to support online socializing \cite{SecondLife}. As of 2021, this community was reported to have 64.7 million active users \cite{SecondLifeActiveUsers}. To enhance the accessibility of this virtual community, Folmer et al. \cite{folmer2009textsl} designed a command-based client so that PVI can type text commands to query information, navigate, and interact with the virtual world by using keyboards. A commercial text-based client, Radegast, has also been released to enable PVI to use Second Life \cite{Radegast1}. 

Besides Second Life, accessibility features have been added to other mainstream virtual worlds for PVI \cite{trewin2008powerup, westin2004game, atkinson2006making}. For example, PowerUp was an educational game based on a virtual world, where students learn how to use science and math concepts to solve critical environmental problems and supported several accessibility features for PVI \cite{trewin2008powerup}. Users can use shortcut keys or type in text commands to control their avatars and receive audio feedback from the environments. High magnification was also provided for low vision users. Terraformers \cite{Terraformers} was another virtual world game that was accessible to PVI. In this game, all game objects can generate 3D sound. Audio-based orientation and navigation tools were also supported in this game, such as a sound compass that generates 3D sound to represent north \cite{westin2004game}. 

Some researchers specifically focused on designing accessible navigation techniques in desktop-based virtual worlds, such as the use of audio beacons to convey object position \cite{walker2006navigation, lokki2005navigation, maidenbaum2013increasing}, auditory icons/earcons to identify objects \cite{heuten2006sonification, oliveira2015games}, signals and audio reflections to create a sonar/echolocation-esque system \cite{waters2001bat, wilkerson2010maze, andrade2018echo}, and verbal descriptions of objects reached through list/grid exploration \cite{matsuo2016audible, nair2021navstick}. For example, Walker and Lindsay \cite{walker2006navigation} studied the impact of different types of beacons on guidance or navigation through a virtual space. de Oliveira et al. \cite{oliveira2015games} created a virtual stage and placed instruments within the environment. Participants then used different music tracks to identify and locate instruments on the stage. Maidenbaum et al. \cite{maidenbaum2013increasing} sonificated the distance between the PVI's avatar and the virtual object in front of him to facilitate navigation in a virtual space. Andrade et al. \cite{andrade2018echo} enabled PVI to use echolocation to navigate a desktop-based virtual world, where the user's avatar can produce mouth-click or clap sound by pressing a key on a keyboard and hear the sound reflection from the environment. However, the echolocation method was only used by a small amount of blind people. Recently, Nair et al. \cite{nair2021navstick} designed a game controller-based navigation technique, allowing PVI to look around a virtual world by scrubbing the thumbstick on a game controller to different directions; the system then announced what were in that direction via spatial audio. They then compared the efficacy of their technique compared to menu-based access of object descriptions.

%All accessibility features for desktop-based virtual worlds relied on inputs from desk-mounted devices (e.g., mouse, keyboard) or conventional game controllers. However, such interactions deviated from the natural interactions that people use to explore a real-world space, which can eliminate users' sense of presence in a virtual world.


%Unlike the desktop-based virtual world that requires users to sit in front of a table and use desktop-mounted input devices, the emerging HMD-based VR supports a fully immersive experience by tracking users' head, body, and controllers, allowing them to flexibly walk around and interact with the virtual space in a natural manner. For example, with HMD-based VR, a user can approach a virtual object and pick it up with a controller just like what they do in the real world. Yet, this immersive VR experience is far from accessible. 

In addition to desktop-based virtual worlds, some research effort has been make on addressing the accessibility issues of HMD-based VR for PVI. 
%enabling PVI to interact with the virtual objects and space by intuitively moving their body. 
%Most such work focused on designing novel haptic devices to enable PVI to navigate a VR space. 
For example, Tzovaras et al. \cite{tzovaras2002design} leveraged the CyberGrasp haptic gloves to generate force feedback to a blind user’s fingers, providing the illusion that they are navigating the virtual space with a cane. The researchers further improved the system by asking the user to hold a real cane \cite{tzovaras2009interactive}, with which the system can detect the user’s grasp posture and provide corresponding force feedback through CyberGrasp. 
In the same vein, Zhao created Canetroller \cite{zhao2018enabling}, a wearable haptic VR controller that simulates white cane interaction for blind people in virtual reality. When a user sweeps the controller and hits a virtual object, a physical resistance and spatial audio sound effect will be generated to simulate the feedback of a white cane hitting a real object. A follow-up work by Siu et al. \cite{siu2020virtual} further improved the design of the controller by providing three dimensional force feedback. 
%A major downside is that, all existing wearable haptic solutions for VR accessibility are heavy, bulky, and hard to setup, especially for users with visual impairments (Figure \ref{fig:canetroller}). Moreover, navigation is only one task in the complex virtual space. Many other important VR tasks, such as manipulating objects, interacting with virtual menus, remain unexplored. 

Unlike most other work that are targeted at general PVI, Zhao et al. \cite{zhao2019seeingvr} specifically focused on low vision people. They designed SeeingVR, a set of 14 visual and audio augmentations that can be applied to any virtual scenes, such as magnification, edge enhancement, text to speech, and visual highlights on salient objects. Post-hoc plugins and a developer toolkit were developed to enable these tools to be easily applied to various mainstream VR applications. 
%Some augmentations were designed to support specific VR tasks, such as visual search and menu selection. %These accessibility tools can be applied to any mainstream Unity-based VR applications as a \textit{post-hoc} plugin. 
%To increase the generalizability of our tools, we also built a developer toolkit that incorporated all these tools to enable VR developers to apply these accessibility features to their applications directly. 
%However, this work only focused on low vision users who have residual functional vision. Most tools were not applicable for people who have little to no vision. 

All prior research focused on basic VR tasks, such as navigation and object perceptions. However, social VR introduces additional complications with the dynamic and unpredictable avatars in the virtual space, with no research addressing the accessibility of the dynamic avatars for PVI in a social VR context. 

\subsection{Technologies to Facilitate Awareness of People in Social Activities}
While the accessibility of avatars in social VR remains nascent, some prior work has been done to assist PVI in social activities in the real world by enhancing their awareness of the conversational partners in social interactions.

Similar to virtual environments, audio techniques have been used to assist in real world navigation

%In most social situations a lot of important information is encoded visually, usually through visual cues. 
To enhance PVI's awareness of people and their non-verbal behaviors in social activities, various wearable or handheld assistive technologies have been developed. These technologies came in a variety of forms, including smartphone applications \cite{zhao2018face}, belts\cite{mcdaniel2008using, buimer2018conveying}, gloves \cite{krishna2010vibroglove, krishna2008systematic}, headband \cite{qiu2016designing, morrison2021peoplelens}, glasses \cite{anam2014expression, terven2014robust}, and wearable cameras \cite{gade2009person, terven2014robust}. For example, Krishna et al. \cite{krishna2008systematic} created a haptic glove called VibroGlove that allowed PVI to understand facial expressions of a conversation partner. The glove consisted of several vibration motors mounted on the back of each finger that was used to present six different emotions (i.e., anger, disgust, happiness, fear, surprise, and sadness) through vibration patterns. These patterns were designed based around the shape of the mouth and eye area of each facial expression. %Similarly, Buimer et al. \cite{buimer2018conveying} combined a head-mounted camera and a haptic belt to relay the same six facial expressions. The camera captured a live video feed of individuals that the software FaceReader 6™ would analyze to detect faces and facial expressions. These facial expressions were then conveyed to the user by a series of vibrating motors in the belt, where each motor represented a different emotion with more positive ones positioned in the front.  
Anam et al. \cite{anam2014expression} used Google glasses to track faces and communicate social signals (i.e, facial features, behavioral expressions, body postures, and emotions) of surrounding people to the PVI verbally. %The Google glasses used a built-in camera to capture these social signals, which were analyzed and then reported back to the PVI through speech audio feedback using a Text-to-Speech service.
%Besides recognizing people, systems have been designed to convey the nonverbal behaviors of surrounding people to PVI. For example, Terven et al. \cite{terven2014robust} created a system of detecting head gestures(i.e, nods and shakes) through an in-visioned device like glasses or a neck-hung device that would contain a built-in camera.
Morrison et al. \cite{morrison2021peoplelens} used a head-mounted device to provide spatial identifyin audio to assist blind children with gaze direction and mental mapping of surrounding people. Another example was Tactile Ban prototyped by Qiu et al. \cite{qiu2016designing}, which used tactile feedback to provide the feeling of other people's gazes onto the PVI. Tactile Ban was a wearable headband where gaze signals were mapped to the vibration signals embedded in the band. The band had two vibrate patterns based on if a person glanced at the PVI or if their gaze was fixated on them currently.

However, these prior works have focused on providing information about the environment with their apparatus as a primary focus for users. They did not explore how to enhance PVI's peripheral awareness (a secondary task) of surrounding human dynamics in a complex social activities, such as approaching or conversing with someone, where they cannot only focus on operation of the device or technique. 

There has been prior work done to facilitate peripheral awareness during collaborative tasks through visual \cite{sideshow, sakashita2022remote} or audio \cite{jung2008sound, kilander2002ambient, das2022, lee2022collab} cues. For example, Lee et al. designed the CollabAlly browser extension, which provided blind users with accessible audio feedback and navigation of content or comment changes. However, visual cues for peripheral awareness are not accessible to PVI. For the work utilizing audio cues, they do not design for the unique challenges posed by a social context. Compared to collaborative tasks which allow for asynchronous interactions, social VR requires immediate response for the dynamic interactions. Thus a different design is needed to adequately facilitate peripheral awareness on the social context.

In our research, we seek to address this gap by designing audio-based awareness techniques, focusing on the social VR context.



==> Sections/2-Related_Work.tex <==
\section{Related Work}
\TODO{rewrite. this paragraph is a summary of the related work session, instead of our contribution.}
Our contributions to this ever-growing research area target the social aspects of Virtual Reality that have yet to be explored in-depth. In VR individuals with visual impairments need other forms of feedback that those sighted do not. A user in a virtual space with sight can view the avatars around them to communicate, however those with visual impairments cannot. We propose multiple audio notification and text-to-speech feedback sounds that are customizable to provide impaired users with awareness needed to communicate in a Virtual World. 

\subsection{The Virtual World and Visual Impairments}
\TODO{The title needs to be more specific. virtual world and virtual impairments do not tell much about the relationship there.}
\TODO{Needs to define virtual world. and i would recommend we use virtual reality instead of virtual world if you don't want to distinguish them. They do not really mean the same thing from some aspects.}
As technology integrates more into society the use of assistive technology is more available to those that need it. When one thinks of assistive technologies they often refer to those that help navigate everyday tasks like Audio based GPS’s \cite{loomis2001gps}, NavCog\cite{ahmetovic2016navcog}, or Sensory Substitution Devices\cite{hamilton2016always}, how to build assistive technologies like icare \cite{panchanathan2003icare}that performed a user-centric approach to determine the vital design choices of assistive devices, or those that enhance current assistive technologies, such as VizWiz \cite{dognin2020image} a dataset of images taken by the visually impaired and captioned to improve assistive image captioning systems. \TODO{this paragraph is a bit too broad about general accessibility research, not highly relevant. consider removing.}

However, with the use of Virtual Reality \TODO{"use of virtual reality" -> virtual reality} becoming more prevalent current research has shifted to include technologies used for entertainment purposes like games. At first, techniques used for creating everyday assistive technologies were applied to games, but this did not produce great results\cite{archambault2008towards} motivating research to create its own accessibility strategies for games. \TODO{by reading this sentence, i cannot tell what this research is about. How did they apply tech to games, and what results they achieved?}

To fully understand what a person with visual impairment would need to play a game, studies have focused on the elements that allow those with impairments to interact with games tailored to the impaired \cite{andrade2020introducing}. Some of these major elements are interacting with the virtual world and navigating it. These core mechanics propose challenges to those with impairments and are present in the majority of games. The element of navigation has been widely studied, haptic feedback is used to compliment most navigational tasks, since the visual impaired rely on hearing and touch \cite{kaklanis2009haptic} \cite{huang2010exploration} \cite{iglesias2004computer}. Other than haptic, applications will use audio\cite{dunai2010real}, recent work Navstick created an audio-based tool for navigating the virtual world to allow exploration\cite{nair2021navstick}.  Other smaller features that have been investigated, but have not been the primary focus, some of these include font customization, orientation tools, and self-voicing text-to-speech output which can be found in PowerUp\cite{trewin2008powerup} a virtual educational game that boasted accessibility features. While most of these games are made for educational/entertainment they are not always,since virtual games can simulate the real world, they can provide other benefits. Sea Hero Quest \cite{coutrot2019virtual} a mobile app was used to predict the navigation abilities of individuals in real-life to help diagnose those with Alzheimer’s and Dementia.

Individuals with impairments often desire to play games made for the sighted and awareness for this growing group is apparent\cite{andrade2019playing} Notable games that have been created with the sole purpose of bridging the gap in game accessibility are Terraformers \cite{westin2004game}one of the earliest creations focused on creating an visual/audio hybrid that could be played by those with sight and impairments.A more recent work ShadowRine\cite{matsuo2016audible} which used visual, auditory, and tactile senses to a create a barrier-free game with a map editor tool for developers with impairments.

\subsection{Social Interaction with Visual Impairments}
\label{sec:Social Interaction with Visual Impairments}
The use of assistive technologies in social situations has grown over the years, with social media increasing the rate of social interactions since it can simulate everyday face-to-face communications and is used in the workplace\cite{wentz2011separate}. Those with visual impairments often are hindered in social situations due to difficulty recognizing non-verbal ques\cite{krishna2008systematic} \cite{qiu2015nonverbal}like gazes\cite{qiu2016mode}, faces, body gestures, and eye-contact. To simulate gaze, eye-contact and facial expressions in real-world settings\cite{qiu2018hci} research has used camera mounted glasses\cite{krishna2010assistive} or haptic motion sensor belts\cite{mcdaniel2008using}. Other approaches include accessibility Bot\cite{zhao2018face}, a Facebook Bot that uses computer vision to identify facial expressions and individuals in photos or web based applications to enhance communications\cite{nishimoto2008analysis}. 

Other concerns in social environments are privacy and how assistive technology is perceived. Individuals with impairments have unique privacy and security concerns like bystanders overhearing conversations and shoulder-surfing\cite{ahmed2015privacy}.They also have a different outlook on how they might be perceived when using an assistive technology, which was found to effect self-efficacy and self-confidence\cite{shinohara2016self}.

The emotional aspects for the visual impaired during social interactions have been greatly documented for different populations. Visual signals are often misunderstood and require designs of these signals to include positive meaning for the user to perceive. \cite{qiu2015nonverbal} The amount of participation in daily activities directly correlates to social roles \cite{desrosiers2009participation} and having a negative social problem solving orientation can predict depression and emotional distress\cite{dreer2005social}. 

\subsection{Virtual Social Interaction}
With the development of virtual reality, the possibility to virtually experience social interaction is  expanding. This growing area of research centers on how users present themselves \cite{freeman2021body}in virtual reality, this tends to refer to the avatars they create. These avatars share similarities to our real life counterparts frequently having their own embodiment, context, and spatial proximity\cite{mennecke2010embodied}. Even though these avatars might share these properties they don’t always line up with our real-life expectations. Personal space which has been found to cause anxiety when someone invades it in real-life and can differ based on gender is not replicated in the virtual space\cite{nassiri2010human}.  However, other aspects do, work has shown participants when performing a task either virtually or in real life while accompanied by others are inhibited\cite{zanbaka2007social}. 

Because avatars play immense role in VR, the amount of customization and control a user has over them affects the embodied experience\cite{kolesnichenko2019understanding}. The realism of the avatar is critical to the development of social environments, work has found that high avatar realism increases copresence while decreasing self-disclosure\cite{bailenson2006effect} and can be beneficial in certain settings like distance learning and therapy. Just like real world social interactions these avatars that embody us have the ability to perform non-verbal actions, which can create complications as mentioned in \ref{sec:Social Interaction with Visual Impairments}. Exploring the type, usefulness, and when these non-verbal ques are  performed is key to advancing VR\cite{maloney2020talking}. Currently users lack control over ambient aspects of nonverbal communication such as posture, pose, and social status\cite{tanenbaum2020make} only furthering obstacles.


Early work determined 20 user embodiment design issues for virtual communication a few of them are: presence, location, identity, gesture, facial expression, voluntary versus involuntary expression, degree of presence, reflecting capabilities, and physical properties, \cite{benford1995user} which share striking similarities to the current design choices for avatars in VR. While the focus on avatars and embodiment is important, other problems in the virtual social space have been worth looking at such as turn taking in conversations, the overall participation in the virtual environments \cite{bowers1996talk}, and the privacy of users in them. For privacy users often feel comfortable to disclose personal information and admit that doing so is an inevitable trade-off.\cite{maloney2020anonymity} \todo{Add this last sentence to the previous one or remove it entirely?}


\begin{comment}
\section{Related Work} [Rough Rough Draft]
Maybe put what our work contributes here?? Or how VR accessibility connects with social interaction in an overall fashion.[TODO: Change lots of Wording, add more details to certain references make things more cohesive]

\subsection{Virtual World Accessibility}
Making the online space accessible for those that have impairments has been looked at since virtual spaces have existed. Video games is one of the first uses of virtual spaces and presents a challenge for those that have a need for accessibility functions. These needs are defined by what a person with visual impairment interacts with in these digital worlds\cite{andrade2020introducing}.Individuals with impairments need these extra mechanics to navigate these virtual worlds. Terraformers was one of the first ever efforts to make a game that was accessible for those with low vision and the average users by using spacial sound and voice feedback \cite{westin2004game}. Research on navigation in the virtual world is plentiful such as \cite{nair2021navstick} which allows the user to explore the world around them by a joystick were they hover over any object and can hear the descriptions of the object. Human wayfinding in the physical world can be applied to construct aids for navigation in virtual worlds as well, such as spacial audio cues,  audio feedback, and how someone navigates the real world environment\cite{darken1996wayfinding}.


\subsection{Social Interaction}
Most recent research covers how individuals with impairments navigate online spaces, making the mechanics of such online spaces more  accessible, or on the non-verbal communication in large multiplayer online games which include 2D/3D virtual worlds \cite{maloney2020talking}. The social aspect is often overlooked and the majority of research that considers social interaction for those impaired , focuses only on the real world. The social aspect in the virtual and real world are important when it comes to conversing, often those with impairments struggle to recognize facial ques \cite{krishna2008systematic}. Past work has looked at developing apps to help those with impairments notice social ques while in a conversation \cite{zhao2018face}. This means they struggle to see gazes or eye contact in social settings, and researchers try to design gaze simulations for those individuals \cite{qiu2018hci}. Not only are people worried about missing social ques they are concerned with those around them that is not in their social activities. Impaired people struggle to protect their privacy in the physical world and online world(e.g., bystanders overhearing private conversations) \cite{ahmed2015privacy}. In virtual worlds your avatar embodies your physical self, there is concern for spacial proximity between yourself and others applies to your virtual self \cite{mennecke2010embodied}  \cite{nassiri2010human} \cite{kolesnichenko2019understanding} \cite{freeman2021body}
\end{comment}
